Probing dynamics and thermal properties inside molecular tori with CO rovibrational absorption lines

A recent hydrodynamic model, "radiation-driven fountain model" (Wada et al. 2016), presented a dynamical picture that active galactic nuclei (AGNs) tori sustain their geometrical thickness by gas circulation around AGNs, and previous papers confirmed that this picture is consistent with multi-wavelength observations of nearby Seyfert galaxies. Recent near-infrared observations implied that CO rovibrational absorption lines ($\Delta J=\pm1$, $v=0-1$, $\lambda \sim 4.7$ $\mathrm{\mu m}$) could probe physical properties of the inside tori. However, the origin of the CO absorption lines has been under debate. In this paper, we investigate the origin of the absorption lines and conditions for detecting them by performing line radiative transfer calculations based on the radiation-driven fountain model. We find that CO rovibrational absorption lines are detected at inclination angles $\theta_\mathrm{obs} = 50-80$ $^{\circ}$. At the inclination angle $\theta_\mathrm{obs} = 77$ $^{\circ}$, we observe multi-velocity components: inflow ($v_\mathrm{LOS}=30$ $\mathrm{kms^{-1}}$), systemic ($v_\mathrm{LOS}=0 \, \mathrm{kms^{-1}}$), and outflows ($v_\mathrm{LOS}=-75,\, -95,$ and $-105$ $\mathrm{kms^{-1}}$). The inflow and outflow components ($v_\mathrm{LOS}= 30$ and $-95$ $\mathrm{kms^{-1}}$) are collisionally excited at the excitation temperature of $186$ and $380$ K up to $J=12$ and $4$, respectively. The inflow and outflow components originate from the accreting gas on the equatorial plane at $1.5$ pc from the AGN center and the outflowing gas driven by AGN radiation pressure at $1.0$ pc, respectively. These results suggest that CO rovibrational absorption lines can provide us with the velocities and kinetic temperatures of the inflow and outflow in the inner a-few-pc regions of AGN tori, and the observations can probe the gas circulation inside the tori.

==> af_discussion2.tex <==
\subsection{Possibilities of future observations for observing CO absorption lines} \label{sec:discuss2}
In Section \ref{sec:result1}-\ref{sec:result4}, we investigate the origin of CO rovibrational absorption lines and the conditions for observing CO rovibrational absorption lines and find that CO rovibrational absorption lines can trace the gas dynamics and the physical properties in the inner few-pc region of molecular tori at incliation angles of $\obs = 50-80 \, ^{\circ}$.
However, 
Here, we discuss objects in which CO rovibrational absorption lines are observed.

\citet{2018PhDT.......191B} investigated CO rovibrational absorption lines in 48 galaxies using low-spectroscopic data of AKARI and extracted physical properties from 33 galaxies.
He found that CO absorption line originates from the gas with high excitation temperature $T_\mathrm{ex} = 100-1000$ K, though he did not decompose each velocity component and each absorption line at each rotational level due to low-spectroscopy.

%Also, he investigated the dependence of the depth of CO absorption line on the IR luminosity of each galaxy.
Also, he found that objects with higher infrared luminosity, such as ULIRGs, show the deeper absorption of the CO absorption lines.
A possible interpretation of this phenomenon is the dependence of the infrared luminosity on the torus structure.
In section \ref{sec:result}, we show that the distributions of dust temperature and the thermal emission depend on the the torus structure.
If we consider a structure where AGN is more covered by a torus, the UV radiation from AGN is more efficiently converted to infrared radiation and show strong infrared luminosity.
Thus, it is expected that, in such objects, more CO molecules cover the thermal emission from hot dust as a background source, and the CO absorption lines show strong absorption.

\citet{Lutz2004} also investigated CO rovibrational absorption lines in 31 galaxies using low-spectroscopic data of ISO and found no significant detection in the all galaxies, even type-2 galaxies.
Our result is consistent with this result.
We find that the thermal emission from the hot dust, a background source, is perfectly self-shielded by surrounding cold dust at a inclination angle $90 \, ^{\circ}$, and thus it is difficult to observe CO rovibrational lines.

%\subsection{Comparisons with observations}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%In previous sections, we made mock spectroscopic observations for  CO rovibrational absorption lines and observe five velocity components.
%Besides, we found that CO molecules are transited radiatively between the rotational levels in the most region of the molecular torus.
%That means LTE assumption is not good for AGN molecular tori. 
%Here, we compare the excitation states of each component with those of observational result qualitatively \citep{Onishi2021}.
%We note that we use different physical model from the observation target, a ULIRG IRAS08572+3915.
%on a seyfert galaxy, circinus galaxy but the observation target is a ULIRG, IRAS08572+3915.

%\citet{Onishi2021} observed a ULIRG, IRAS08572+3915, and decomposed CO rovibrational absorption lines into five velocity components as described in sec.\ref{sec:intro}.

%\subsection{Depth of absorption lines}
%Here, we compare the line depth of rovibrational absorption P(4) 
%\subsection{Excitation states of velocity components}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Possibility of IR pumping for CO excitation}

